SHIFT3D: Synthesizing Hard Inputs For Tricking 3D Detectors

We present SHIFT3D, a differentiable pipeline for generating 3D shapes that are structurally plausible yet challenging to 3D object detectors. In safety-critical applications like autonomous driving, discovering such novel challenging objects can offer insight into unknown vulnerabilities of 3D detectors. By representing objects with a signed distanced function (SDF), we show that gradient error signals allow us to smoothly deform the shape or pose of a 3D object in order to confuse a downstream 3D detector. Importantly, the objects generated by SHIFT3D physically differ from the baseline object yet retain a semantically recognizable shape. Our approach provides interpretable failure modes for modern 3D object detectors, and can aid in preemptive discovery of potential safety risks within 3D perception systems before these risks become critical failures.

==> Rendering.tex <==
\subsection{Rendering SDF Assets with Realistic Occlusions in the Log Scenes}
Due to the large number of LiDAR points in a scene (e.g. 100k to 200k in a scene in Waymo Open Dataset), processing all of them at once is memory-intensive. To overcome this, we select a set of active points from the log scene that may change when the SDF asset is added. The active points are chosen in the form of a cone, where the direction of the cone is determined by the intended placement of the asset. If the asset is meant to be placed beyond a certain distance from the LiDAR sensor, we can mask off points within a certain distance to the sensor to create a truncated cone as the region of interest (ROI). We assume that the SDF asset will always be added in the ROI. It is essential to note that this region of interest is in the original log scene without SDF assets added. Each LiDAR sensor and its corresponding point cloud has their own ROI. If multiple sensors are present, the union of the selected points is used. This technique can significantly reduce the number of active points to less than 20k, allowing for more efficient processing. Points outside the ROI are inactive and are kept as they are.

To determine whether an active point in the region of interest (ROI) belongs to the SDF asset or not after it is added, we draw a straight line from that point to LiDAR sensor. Next, we sample points along the line and calculate their respective SDF values.
If all the sampled points have SDF values greater than 0, then the original point in the ROI is considered off the asset and is kept as it is. 
If any sampled points have SDF values less than 0, the original point in the ROI is occluded and requires further processing. In such cases, we perform a binary search to find the intersection point of the straight line and the SDF surface, bringing the occluded point to the resulting point on the asset.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/ROI.pdf}
    \caption{Rendering SDF Assets with Realistic Occlusions in the Log Scenes}
    \label{fig:roi}
    % link: https://docs.google.com/drawings/d/1oZ8Z5ZepQ_gbc4gu0J96Z_tnEWwg_YIMKHDxnPexwvA/edit?usp=sharing
\end{figure}

\subsection{Realism Constraints}

\subsubsection{No Overlapping with the Log Scene}
To ensure that the SDF asset does not overlap with existing objects in the log scene, we need to verify that all the points in the original log scene have an SDF value greater than 0. If any of the original points have an SDF value less 0, that indicates that the point is inside the SDF asset, and the SDF asset would overlap with an object in the log scene. 
\subsubsection{Asset Touches the Log Scene}
We aim to ensure that the SDF asset is not suspended in mid-air. To achieve this, we need to ensure that there is at least one point in the original scene with an SDF value less than a predefined small positive number $\epsilon_{\text{float}}$. This ensures that the point is in contact with the SDF surface, and the SDF asset is placed on a surface rather than floating in the air. 
\subsubsection{Asset Not Occluded}
After determining where to place the asset, we run ray casting to generate point cloud on the asset. If there are no points landing on the asset, we determine that the asset is occluded. 

==> baseline_objects_plot.tex <==
\begin{figure*}
       \centering

\begin{subfigure}[b]{0.196\textwidth}
\includegraphics[width=\textwidth]{figures/threshold_recall/ef6Coupe.png}
\caption{Coupe}
\end{subfigure}
%
\begin{subfigure}[b]{0.196\textwidth}
\includegraphics[width=\textwidth]{figures/threshold_recall/dcaSportsCar.png}
\caption{Sports Car}
\end{subfigure}
%
\begin{subfigure}[b]{0.196\textwidth}
\includegraphics[width=\textwidth]{figures/threshold_recall/df7SUV.png}
\caption{SUV}
\end{subfigure}
%
\begin{subfigure}[b]{0.196\textwidth}
\includegraphics[width=\textwidth]{figures/threshold_recall/e9aConvertible.png}
\caption{Convertible Car}
\end{subfigure}
%
\begin{subfigure}[b]{0.196\textwidth}
\includegraphics[width=\textwidth]{figures/threshold_recall/ee9BeachWagon.png}
\caption{Beach Wagon}
\end{subfigure}
\caption{The reconstruction of baseline objects from the trained SDF models. All vehicles belong to the ``Automobile" category of the ShapeNet dataset~\cite{chang2015shapenet}. }
\label{fig:original_mesh}
    \end{figure*}

==> problem_formulation.tex <==
We approach the problem by formulating it as a semantic adversarial example generation. To do this, we have developed an adversarial asset generator that adds assets to a LiDAR log scene. The generator uses a SDF to model the 3D shape of the assets and performs ray casting to render their point cloud, which is then added to the log scene. The generator allows us to control the translation, rotation, size, and shape encoding of the assets, as well as to render realistic occlusions based on the existing point cloud and sensor positions in the scene. To search for the optimal adversarial assets, we explore the parameters of position, rotation, and shape. 
To make the process efficient and effective, we have made our pipeline end-to-end differentiable, allowing us to calculate gradients with respect to the parameters and shape encoding of the adversarial asset generator. Our ultimate goal is to generate adversarial assets that meet two criteria: they should significantly reduce the performance of perception models, yet remain semantically valid and realistically shaped. 
\subsection{Requirements}
There are two requirements (goals) for the generated assets and scene:
Long tail/Adversarial: The perception models' performance on the generated dataset should significantly deteriorate in comparison to their performance on natural examples.
Realism: The generated examples should be both semantically valid and realistic. Semantically valid scenes are acceptable even if they differ from the original seed scenes, but measuring the realism of such generated scenes could be challenging. It's not necessary for the generated scenes to resemble the original scene.
\subsection{What We Can Control?}
We generate the adversarial asset by controlling the following two sets of input parameters:
\begin{enumerate}
 
\item Latent Shape Encoding (parameterized as $\B z$). This determines the actual shape of the assets generated. It is similar to the embedding vector in generative models such as GAN or VAE.
\item Rigid Body Transformation (parameterized as $\B\theta$): This determines where and how the assets will be placed in the scene. It gives the rotation angle, $(x, y, z)$ position, and the size of the assets.
\end{enumerate}
\subsection{Differentiable Search}
To generate adversarial assets, we need to search in two parameter spaces. To make the search process efficient and effective, we require a differentiable pipeline. This allows us to backpropagate through the perception model, point cloud, and adversarial asset generator, all the way to the Rigid Body Transformation $\mathbf{\theta}$ and latent shape encoding $\B z$.

